Non-perturbative Renormalization Constants using Ward Identities

We extend the application of vector and axial Ward identities to calculate $b_A$, $b_P$ and $b_T$, coefficients that give the mass dependence of the renormalization constants of the corresponding bilinear operators in the quenched theory. The extension relies on using operators with non-degenerate quark masses. It allows a complete determination of the $O(a)$ improvement coefficients for bilinears in the quenched approximation using Ward Identities alone. Only the scale dependent normalization constants $Z_P^0$ (or $Z_S^0$) and $Z_T$ are undetermined. We present results of a pilot numerical study using hadronic correlators.

==> Makefile <==
# %auto-ignore
MAINFILE=  wi.tex
TEXFILES=  
AXISFILES= 
FIGFILES=
EPSFILES=

#########################################################################
# List of all the sources
SOURCES= Makefile ${MAINFILE} ${TEXFILES} ${AXISFILES} ${FIGFILES} ${EPSFILES}

# List of all postscript figures to be included.
PSINCLUSIONS= ${AXISFILES:.ax=.eps} ${FIGFILES:.fig=.eps} ${EPSFILES}

# what is to be made by default
all: ${MAINFILE:.tex=.ps}

# re-dvips if any of these change
${MAINFILE:.tex=.ps}: ${MAINFILE:.tex=.dvi} ${PSINCLUSIONS}

# re-latex if any of these change
${MAINFILE:.tex=.dvi}: ${MAIN} ${TEXFILES} ${PSINCLUSIONS}

# Never try to `make' any of the sources
${SOURCES}:;

# The rest of them do not have any `extra' dependencies, i.e. a.x depends 
# obviously depends on a.y if a.x is to be created from a.y.

.PHONY: clean realclean
# clean removes ~ aux log and tmp files
clean:
	rm -f *~ *.aux *.log *.tmp
# real clean removes everything but sources and final products
realclean: clean
	rm -f ${AXISFILES:.ax=.ps} ${AXISFILES:.ax=.eps} ${FIGFILES:.fig=.eps}

########################################################################
# General rules of how to build something from something else.
.SUFFIXES: .ps .eps .dvi .tex .ax .xy .fig

# If .fig exists that is how to create eps.
%.eps: %.fig
	fig2dev -L ps $< > $@

# else try to create it from ps
%.eps: %.ps
	sed -e "s/%%BoundingBox: 0.*/`psbbox $<`/" $< > $@ 

# If .ax or .xy exist, that is the source of the .ps file
%.ps: %.ax
	xyplot $< | epsplot > $@
%.ps: %.xy
	xyplot $< | epsplot > $@

# else look for a dvi file.
%.ps: %.dvi
	dvips -z -o $@ $<


# dvi is always created from tex.
%.dvi: %.tex
	latex $< && latex $< && latex $<

##################################################################

submission: ${SOURCES} ${PSINCLUSIONS}
	(echo "."; \
	 echo "${SOURCES} ${PSINCLUSIONS}" ; \
	 echo "submission") | uufiles -gz -9


